HARP: A Taxonomy for Heterogeneous and Hierarchical Processors for Mixed-reuse Workloads

Artificial intelligence (AI) application domains consist of a mix of tensor operations with high and low arithmetic intensities (aka reuse). Hierarchical (i.e. compute along multiple levels of memory hierarchy) and heterogeneous (multiple different sub-accelerators) accelerators are emerging as a popular way to process mixed reuse workloads, and workloads which consist of tensor operators with diverse shapes. However, the space of hierarchical and/or heterogeneous processors (HHP's) is relatively under-explored. Prior works have proposed custom architectures to take advantage of heterogeneity to have multiple sub-accelerators that are efficient for different operator shapes. In this work, we propose HARP, a taxonomy to classify various hierarchical and heterogeneous accelerators and use the it to study the impact of heterogeneity at various levels in the architecture. HARP taxonomy captures various ways in which HHP's can be conceived, ranging from B100 cores with an "intra-node heterogeneity" between SM and tensor core to NeuPIM with cross-depth heterogeneity which occurs at different levels of memory hierarchy. We use Timeloop mapper to find the best mapping for sub-accelerators and also modify the Timeloop cost model to extend it to model hierarchical and heterogeneous accelerators.

==> tables/old/config.tex <==
\begin{scriptsize}
    \begin{table}[h!]
\begin{scriptsize}
    
  \begin{center}
  \caption{Configurations for workloads and architecture} 
  %\Rav{There is space for remarks too if needed}}
  %\TK{@Raveesh - by x do you mean you can do either s or t for that dimension? So does that mean each row is actually multiple datapoints? Thats confusing.}\Rav{It means that the datapoint that we choose for evaluation of that dataflow can have varaible tile sizes for dimension marked by X. S and T on the other hand mean that its NECESSARILY spatial or temporal}}
  \label{table:config}
  \begin{centering}
  \begin{tabular}{|l|l|}
    \hline
    \textbf{Parameter} & \textbf{Value}  \\
    \hline
    %Seq & $V\times F$ & $t_{AGG}+t_{CMB}$\\
    %\hline
    Bytes per word/element & 1B (8 bits)\\\hline
    PE array size & 32$\times$32\\ 
    \hline
    PE dot product size\footnote{No reduction for grouped convolutions} & 8\\\hline
  %  PE array size at scale (\autoref{fig:scale}) & 256$\times$256\\ \hline
  % PE dot product size at scale (\autoref{fig:scale}) & 32\\\hline
    SRAM capacity & 1MB \\\hline
 %  SRAM capacity at scale (\autoref{fig:scale}) & 8MB\\ \hline
%    Off-chip bandwidth & \\\hline
 %   On-chip bandwidth & \\\hline
  %  Inter-cluster bandwidth & \\\hline
   Memory bandwidth & 256 GB/s\\\hline
 %   Memory bandwidth at scale (\autoref{fig:scale}) & 1TB/s\\\hline
    %Total L2 capacity & 32MB\\ \hline
    %Total L3 capacity & 256MB\\ \hline
  \end{tabular}
\vspace{-3mm}
\end{centering}
\end{center}
\end{scriptsize}

\end{table}
\end{scriptsize}

==> tables/old/config_backup.tex <==
\begin{scriptsize}
    \begin{table}[h!]
\begin{scriptsize}
    
  \begin{center}
  \caption{Configurations for workloads and architecture} 
  %\Rav{There is space for remarks too if needed}}
  %\TK{@Raveesh - by x do you mean you can do either s or t for that dimension? So does that mean each row is actually multiple datapoints? Thats confusing.}\Rav{It means that the datapoint that we choose for evaluation of that dataflow can have varaible tile sizes for dimension marked by X. S and T on the other hand mean that its NECESSARILY spatial or temporal}}
  \label{table:config}
  \begin{centering}
  \begin{tabular}{|l|l|}
    \hline
    \textbf{Parameter} & \textbf{Value}  \\
    \hline
    %Seq & $V\times F$ & $t_{AGG}+t_{CMB}$\\
    %\hline
    Bytes per word/element & 1B (8 bits)\\\hline
    PE array size & 32$\times$32\\ 
    \hline
    PE dot product size\footnote{No reduction for grouped convolutions} & 8\\\hline
  %  PE array size at scale (\autoref{fig:scale}) & 256$\times$256\\ \hline
  % PE dot product size at scale (\autoref{fig:scale}) & 32\\\hline
    SRAM capacity & 1MB \\\hline
 %  SRAM capacity at scale (\autoref{fig:scale}) & 8MB\\ \hline
%    Off-chip bandwidth & \\\hline
 %   On-chip bandwidth & \\\hline
  %  Inter-cluster bandwidth & \\\hline
   Memory bandwidth & 256 GB/s\\\hline
 %   Memory bandwidth at scale (\autoref{fig:scale}) & 1TB/s\\\hline
    %Total L2 capacity & 32MB\\ \hline
    %Total L3 capacity & 256MB\\ \hline
  \end{tabular}
\vspace{-3mm}
\end{centering}
\end{center}
\end{scriptsize}

\end{table}
\end{scriptsize}

==> tables/old/noc.tex <==
\begin{scriptsize}
\begin{table}[h]
\begin{scriptsize}
    
    \centering
      \caption{Summary of mesh bottlenecks observed in~\autoref{fig:fine_grained_patterns}-\ref{fig:2Dinterleaving}.}
    \label{table:noc}
    \begin{tabular}{|c|c|c|}
            \hline

        \textbf{Cause} & \textbf{Effect} & \textbf{Prevalent in} \\\hline
       Many long overlapping paths  & High Congestion & Blocked 1D and 2D \\\hline
       Many long overlapping paths  & High hop energy & Blocked 1D and 2D\\\hline
       Extra BW for skip connections & High congestion & All organizations \\\hline
        Extra hops with skip connections & High hop energy & All configurations \\\hline
        Routing in multiple directions & Higher hop energy & 2D organizations\\\hline
    \end{tabular}
  \end{scriptsize}
\end{table}
\end{scriptsize}

==> tables/old/related_pipeline.tex <==
\begin{table}[ht!]
\begin{scriptsize}
\begin{center}
\caption{Related work table showing prior works on inter-layer pipelining. Regarding orange checkmark, - 1) TileFlow canonically supports variable depth but fixes it within an application, and 2) HyGCN has two granularities.%\TK{this table still says violin!}
}
\label{tables:related-pipeline}

{%\tt
\begin{tabular}{|c|c|c|c|}\hline
 \textbf{Prior Work} & \textbf{Variable} & \textbf{Variable} & \textbf{Contibution}\\
 & \textbf{Depth} & \textbf{Granularity} &
 \\\hline

 Atomic  & \greencheck & \redcheck & Inter-operation\\
 Dataflow~\cite{atomic-dataflow} & & & mapper
 \\\hline

 Stream~\cite{genetic-pipeline} & \redcheck & \greencheck & Heterogeneous \\
 & & & Dataflow Framework\\\hline

  HyGCN~\cite{yan2020hygcn} & \redcheck & \orangecheck & Accelerator \\\hline

  EnGN~\cite{liang2020engn} & \redcheck & \redcheck & Accelerator\\\hline
   OMEGA~\cite{garg2021understanding} & \redcheck & \greencheck & Cost model  \\\hline

   TANGRAM~\cite{tangram} & \greencheck & \redcheck & New dataflow  \\\hline

    FusedCNN~\cite{fusedcnn} & \redcheck & \redcheck  & Accelerator  \\\hline

    SET~\cite{isca-pip} & \greencheck & \redcheck & Mapper  \\\hline
 
TileFlow~\cite{tileflow} & \orangecheck & \greencheck & Mapper \\\hline

SIMBA~\cite{simba} & \greencheck & \redcheck & Mapper\\\hline

    \DataflowName &  \greencheck & \greencheck & Spatial organization,  \\    
    &&& NoC and Dataflow\\\hline




\end{tabular}
}
\end{center}
\end{scriptsize}
\vspace{-0.1cm}
%'Sp' prefix implies support for zero skipping. IP=Inner Product, OP=Outer Product, Gust=Gustavsons}
\vspace{-0.45cm}
\end{table}

==> tables/old/related_work.tex <==
\begin{table}[ht!]
\begin{scriptsize}
\begin{center}
\caption{Related work table showing prior works related to mapping exploration and multi-layer acceleration.}
\label{tables:related}

{%\tt
\begin{tabular}{|c|c|c|}\hline
 \textbf{Prior Work} & \textbf{Pipeline} & \textbf{Main Contributions}  \\\hline
 Planaria~\cite{planaria} &  \redcheck  & Multi-tenant accelerator\\\hline
 AI-MT~\cite{AIMT}  & \redcheck  & Multi-tenant accelerator
 %\\ & reduction tree
% & & &
 \\\hline

 GAMMA~\cite{kao2020gamma} &  \redcheck & Mapper

 %\\ & unit
 %& & &
 \\\hline

MAESTRO~\cite{kwon2019understanding} & \redcheck  & Cost model\\\hline

 CoSA~\cite{cosa} &  \redcheck  &  Mapper\\\hline
 
 MAGMA~\cite{magma} &  \redcheck  & HDA Framework \\\hline
 Herald & \redcheck & HDA Framework\\\hline

 Atomic Dataflow~\cite{atomic-dataflow} &  \greencheck  & Intra-operation mapper\\\hline

 Stream~\cite{genetic-pipeline} & \greencheck & HDA Framework\\\hline

  HyGCN~\cite{yan2020hygcn}  & \greencheck  & Accelerator\\\hline

EnGN~\cite{liang2020engn}
 & \greencheck & Accelerator, fine-grained fusion.\\\hline   OMEGA~\cite{garg2021understanding} & \greencheck  &  Cost model\\\hline

   TANGRAM~\cite{tangram} &  \greencheck   & New Dataflow\\\hline

    FusedCNN~\cite{fusedcnn} & \greencheck  & Accelerator\\\hline


SET~\cite{isca-pip} &  \greencheck  & Mapper\\\hline

TileFlow~\cite{tileflow} &\greencheck & Mapper \\\hline


    \DataflowName (This work) &  \greencheck &  NoC and Spatial Organization \\\hline




\end{tabular}
}
\end{center}
\end{scriptsize}
\vspace{-0.1cm}
%'Sp' prefix implies support for zero skipping. IP=Inner Product, OP=Outer Product, Gust=Gustavsons}
\vspace{-0.15cm}
\end{table}
